Efficient Discovery of Actual Causality using Abstraction-Refinement

Causality is the relationship where one event contributes to the production of another, with the cause being partly responsible for the effect and the effect partly dependent on the cause. In this paper, we propose a novel and effective method to formally reason about the causal effect of events in engineered systems, with application for finding the root-cause of safety violations in embedded and cyber-physical systems. We are motivated by the notion of actual causality by Halpern and Pearl, which focuses on the causal effect of particular events rather than type-level causality, which attempts to make general statements about scientific and natural phenomena. Our first contribution is formulating discovery of actual causality in computing systems modeled by transition systems as an SMT solving problem. Since datasets for causality analysis tend to be large, in order to tackle the scalability problem of automated formal reasoning, our second contribution is a novel technique based on abstraction-refinement that allows identifying for actual causes within smaller abstract causal models. We demonstrate the effectiveness of our approach (by several orders of magnitude) using three case studies to find the actual cause of violations of safety in (1) a neural network controller for a Mountain Car, (2) a controller for a Lunar Lander obtained by reinforcement learning, and (3) an MPC controller for an F-16 autopilot simulator.

==> absrefOld.tex <==
\section{Abstraction-Refinement for Causal Models}






% \begin{definition}
	% \emph{Kripke Structures} serve as a conventional model for dynamic finite-state systems.
	% \newline Let \AP\ be a finite set of atomic propositions, a Kripke Structure is a 4-tuple $M = (S,I,R,L)$, where $S$ is a finite set of states, $I \subseteq S$ is a non-empty set of initial states, $R \subseteq S \times S $ is a total transition relation and $L: S \rightarrow 2^{AP} $is a labeling function. 
	% \newline A path in $M$ is an infinite sequence of states $\pi = s_0,s_1,s_2,\dots$ such that $(s_i,s_{i+1}) \in R$ for every $i \in \mathbb{N}$. A trace over \AP\ is an infinite sequence $\tau \in (2^{AP})^w$. We sometimes refer to a trace as a word over $2^{AP}$. A trace property over \AP\ is a set of traces over \AP.
	
	% \end{definition}

% \begin{definition}
	%     A \emph{counterexample} to an LTL formula $\EFE$ in a Kripke structure $K$ is a computation path $\pi = s_0,s_1,s_2,\dots$ such that $\NMOD$. For a state $s_i$ and a variable $v$, the labeling function $L$ of $K$ maps the pair $\langle s_i,v \rangle$ to $\{0,1\}$ in a natural way: $L(\langle s_i,v\rangle) = 1$ if $v \in s_i$, and 0 otherwise.  For a pair $\langle s,v \rangle$ in $\pi$, we denote by $\langle s,\hat{v} \rangle$ the pair that is derived from $\langle s,v \rangle$ by switching the labeling of $v$ in $s$. Let $\pi$ be a path, $s$ a state in $\pi$ and $v$ a variable in the labeling function. We denote $\pi^{\langle s,\hat{v} \rangle}$  the path derived from $\pi$ by switching the labeling of $v$ in s on $\pi$. This definition can be extended for a set of pairs A: we denote $\hat{A}$ the set $\{\langle \hat{s}, v\rangle |\langle s, v\rangle \in A\}$. The path $\pi^{\hat{A}}$ is then derived from $\pi$ by switching the values of $v$ in $s$ for all pairs $\langle s,v \rangle \in A$.
	
	% \end{definition}
	
In this section, we propose our abstraction-refinement technique and its application in reasoning about actual causality, as presented in Section~\ref{sec:smt}.

\subsection{Approximating Causal Models}

The approximate causal models, represented by $O$ and $U$ for \ovr\ and \und\ respectively, 
succinctly capture the breadth and conservatism of the model's estimations.
\begin{itemize}
	\item Concert model: $\ConMod$
	\item Over-approximate model: $\OvMod$
	\item Under-approximate model: $\UnMod$
\end{itemize} 


\begin{definition}
	Given an \ovr\ causal model $\OvMod$, we construct a sequence $O_0 \geq O_1 \geq \dots O_k 
	\geq \mathcal{M}$ of \ovr\, where $O_{i+1}$ (for $0 \leq i < k$) is a refinement of $O_i$, which 
	we compute using \emph{counterexamples}.
	%
	A \emph{counterexample} is a state of $O_{i}$ that is not in $\mathcal{M}$. \todo{change 
		wording}
	%
	\Ovr\ function $\FunOvrV$, that maps \ENDO\ states of $\mathcal{M}$ to \ENDO\ states 
	of $O$. 
	%
	We need two additional functions: $\FunOvrU$, which maps \EXO\  states of 
	$\mathcal{M}$ to \EXO\ states of $O$, and $\hintO$ which maps \ovr\ interventions to \con\ 
	interventions.
	\todo{BB: what about $\mathcal{U}$?} 
\end{definition}

\begin{definition}
	Given an \und\ causal model $\UnMod$, we construct a sequence $U_0 \leq U_1 \leq \dots U_k \leq 
	\mathcal{M}$ of \und, where $U_{i+1}$ (for $0 \leq i < k$) is a refinement 
	of $U_i$, which we compute using \emph{counterexample}. 
	%
	A \emph{counterexample} is a state of $\mathcal{M}$ that is not in $U_{i}$. 
	%
	\Und\ function $\FunUndV$, that maps \ENDO\ states of $\mathcal{M}$ to \ENDO\ states of $U$. 
	%
	We need two additional functions: $\FunUndU$, which maps \EXO\  states of $\mathcal{M}$ to \EXO\ states of $U$, and $\hintU$ which maps \und\ interventions to \con\ interventions.
\end{definition}

\begin{definition}
	Given a set $\mathcal{V}$ of \ENDO\ variables, $\vec{X} \subseteq \mathcal{V}$, and $\vec{x} \in \mathcal{R}(\vec{X})$, let \RST\. 
	%
	Given $\FunOvrV$ define $w_O(\vec{X}\leftarrow \vec{x}) = \vec{Y} \leftarrow \vec{y}$ if $\vec{Y} \subseteq \mathcal{V}_O$, $\vec{y} \in \mathcal{R}_O(\vec{Y})$, and $h_O(Rst(\mathcal{V}_{\mathcal{M}},\vec{x}))=Rst(\mathcal{V}_O,\vec{y})$. 
	%
	It is easy to see that, given $\vec{X}$ and $\vec{x}$, there can be at most one such $\vec{Y}$ and $\vec{y}$. 
	%
	If such a $\vec{Y}$ and $\vec{y}$ do not exist, we take $w_O(\vec{X}\leftarrow \vec{x})$ to be undefined. 
	%
	Let $I_{\mathcal{M}}^{h_O}$ be the set of interventions for which $w_O$ is defined, and let $I_O^{h_O} = w_O(I_{\mathcal{M}}^{h_O})$.
\end{definition}

\begin{definition}
	Given a set $\mathcal{V}$ of \ENDO\ variables, $\vec{X} \subseteq \mathcal{V}$, and $\vec{x} \in \mathcal{R}(\vec{X})$, let \RST\. 
	%
	Given $\FunUndV$ define $w_U(\vec{X}\leftarrow \vec{x}) = \vec{Y} \leftarrow \vec{y}$ if $\vec{Y} \subseteq \mathcal{V}_U$, $\vec{y} \in \mathcal{R}_U(\vec{Y})$, and $h_U(Rst(\mathcal{V}_{\mathcal{M}},\vec{x}))=Rst(\mathcal{V}_U,\vec{y})$. 
	%
	It is easy to see that, given $\vec{X}$ and $\vec{x}$, there can be at most one such $\vec{Y}$ and $\vec{y}$. 
	%
	If such a $\vec{Y}$ and $\vec{y}$ do not exist, we take $w_U(\vec{X}\leftarrow \vec{x})$ to be undefined. 
	%
	Let $I_{\mathcal{M}}^{h_U}$ be the set of interventions for which $w_U$ is defined, and let $I_U^{h_U} = w_U(I_{\mathcal{M}}^{h_U})$.
\end{definition}
In this context, the introduction of a notation termed \emph{allowed intervention} becomes crucial.
%
This notation is essential as certain interventions in the abstract model may lack definition or relevance in a well-defined concrete model. 
%
Consequently, within this framework of definitions, the translation of interventions is not universal; rather, only essential interventions that can be meaningfully mapped are considered.

\iffalse

\input{algo}

\begin{definition}
	If $\FunOvrV$, then $(O,I_O)$ and $(\mathcal{M},I_{\mathcal{M}})$ are $h_O$-cosistent if $h_O$ is surjective, $I_O = w_O(I_{\mathcal{M}})$, and $\dimO$.
\end{definition}

\begin{definition}
	If $\FunUndV$, then $(U,I_U)$ and $(\mathcal{M},I_{\mathcal{M}})$ are $h_U$-cosistent if $h_U$ is surjective, $I_U = w_U(I_{\mathcal{M}})$, and $\dimU$.
\end{definition}

\begin{definition}
	\color{red}
	We Can define the concept of something like $\tau-abstarction$ here but Im not sure about it. 
	
\end{definition}



\subsection{probabilistic Causal Models}

A probabilistic causal model $\mathcal{M} = (S, F, I, Pr)$ is just a causal model together with a probability $Pr$ on contexts $\vec{u}$. 






% \begin{definition}
	%    Let $M_1 = (S_1,I_1,R_1,L_1)$ and $M_2 = (S_2,I_2,R_2,L_2)$ be \emph{Kripke structures} over \AP. A simulation from $M_1$ to $M_2$ is a relation $H \subseteqeq S_1 \times S_2$ such that for every $(s_1, s_2) \in H$:
	% \begin{itemize}
		%     \item[--] $L(s_1) = L(s_2)$
		%     \item[--] For every $(s_1,s_1') \in R_1$ there exists $s_2' \in S_2$ such that $(s_2,s_2') \in R_2$ and $( s_1' , s_2' ) \in H $.
		% \end{itemize}
	% If additionally, for every $s_0 \in I_1$ there exists $s_0' \in I_2$ such that $(s_0,s_0') \in H$, we denote $M_1\leq_{H}M_2$. We denote $M_1\leq M_2$ if $M_1\leq_{H}M_2$ holds for some simulation $H$.
	% \newline \textcolor{blue}{Let $M_1,M_2 $ be two Kripke structures such that $M_1\leq M_2$. Then $M_1 \models M_2$.} 
	% \end{definition}



% \begin{definition}
	%     Given a Kripke structure $M = (S,I,R,L)$ over \AP, we construct an \emph{over-approximations} sequence $O_0 \geq O_1 \geq \dots O_k \geq M$, where $O_{i+1}$ is a refinement of $O_i$, which we compute by using counterexamples. A counterexample is a word $w \in L(O_i)$ yet $w \notin L(M)$. It suffices to consider finite prefixes of $w$, since there is an index $j$ for which $w_0,w_1,\dots,w_{j - 1} \in L(O_i) \backslash L(M)$.
	% \newline We use a sequence of abstraction functions $h_0,\dots,h_k$, each defining an abstract model.
	% \end{definition}



% \begin{definition}
	%     Given $ M = (S, I, R, L)$ over \AP, we construct a sequence of \emph{under-approximations} $U_0\leq U_1\leq\dots \leq U_k\leq M$ via a sequence of abstraction functions using counterexamples. In this case, a counterexample is a word $w \notin L(U)$, yet $w \in L(M)$. Again, we can consider a prefix of $w$.
	% \end{definition}

% \begin{definition}
	%     Given causal model \MOD$=((\mathcal{V},\mathcal{U},\mathcal{R}),F)$ and 
	%     $Y\in\mathcal{U}\cup\mathcal{V}$.  we construct a sequence $O_0 \geq O_1 \geq \dots O_k \geq 
	%     \mathcal{M}$ of \emph{over-approximations}, where $O_{i+1}$ (for $0 \leq i < k$) is a refinement 
	%     of $O_i$, which we compute using counterexamples. \todo{BB: what about $\mathcal{U}$?}
	%  A counterexample is a set $s \in \mathcal{R}(Y_{O_{i}})$ yet $s \notin \mathcal{R}(Y_{\mathcal{M}})$ \todo{BB: should it be $O_{i+1}$ instead of $\mathcal{M}$?}. We use a sequence of abstraction functions $h_{O_{1}},\dots,h_{O_{k}}$, each defining an abstract model. \todo{BB: What do these functions map? they are not well defined.}
	
	% \end{definition}
% \color{blue}
%  \begin{enumerate}
	%      \item fixed the $\mathcal{U}$ problem, now we have Y that is, all variables both \EXO\ and \ENDO
	%      \item No it shouldn't be $O_{i+1}$ cause every time we compare $O_i$ with concrete model to have the counter examples. 
	%      \item These functions are abstract functions that map each under or over approximate to the concrete model. 
	
	
	%  \end{enumerate}
%  \color{black}

% \todo{BB: I don't follow this definition. I tried to understand it by the example in  Sec 4 but I couldn't because the example doesn't use the same notation. }


% \begin{definition}
	%     Given causal model \MOD$=((\mathcal{V},\mathcal{U},\mathcal{R}),F)$ and $Y\in\mathcal{U}\cup\mathcal{V}$, we construct an \emph{under-approximations sequence} $U_0 \leq U_1 \leq \dots U_k \leq \mathcal{M}$, where $U_{i+1}$ is a refinement of $U_i$, which we compute by using counter-examples. A counterexample is a set $s \notin \mathcal{R}(Y_{U_{i}})$ yet $s \in \mathcal{R}(Y_{\mathcal{M}})$. We use a sequence of abstraction functions $h_{U_{1}},\dots,h_{U_{k}}$, each defining an abstract model. 
	% \end{definition}



% \section{Theorem}
% \textbf{Theorem} Given a causal setting \MU\ and its over-approximation $(\vec{O}, \vec{u})$ and under-approximation $(\vec{U}, \vec{u})$, if $\vec{X}= \vec{x}$ is an actual cause for effect $\varphi$ in the $\vec{O}, \vec{U}$, with mapping function $h_U: \mathcal{R}(Y_M)\rightarrow \mathcal{R}(Y_U)$ and $h_O: \mathcal{R}(Y_M)\rightarrow \mathcal{R}(Y_U)$, such that $h_U^{-1}(\vec{x})$ and $h_U^{-1}(\varphi)$ would be the cause and effect in the concrete model.
% \newline \newline \textbf{New Proof} In this proof we need to show that, $\vec{X}=h_U^{-1}(\vec{x})$ is cause of $h_U^{-1}(\varphi)$ in \MU\ that satisfies conditions in \HP\ definition. 
% \begin{itemize}
	%     \item [--] We need to show that $(\mathcal{M},\vec{u}) \models (\vec{X} = h^{-1}_U(\vec{x}))h^{-1}_U(\varphi)$, this is easy to see that if we find a cause and effect in under-approximate abstract, it is is going to be a cause for the concrete model, because in the definition of under-approximate abstract $U\leq $\MOD\ so it is impossible to find a causal relation in $U$ that is not true in \MOD.
	%     \item[--] We need to show that $ (\mathcal{M},\vec{u}) \models (\vec{X} \leftarrow h^{-1}_U(\vec{x}'), \vec{W}\leftarrow h^{-1}_U(\vec{w}_U))\neg h^{-1}_U(\varphi)$, so in other words counterfactual criterion under the \emph{contingency} $\vec{W}\leftarrow h_O^{-1}(\vec{w})$ in abstract model should be observed in concrete model. Same as the first item it is easy to show that if $h_U^{-1}(\vec{x})$ does not happen in the concrete model we are going to see $h_U^{-1}(\varphi)$, and also we need to show that any subset of $\vec{W}$ held constant at some setting $h_O^{-1}(\vec{w})$. As we know $O\geq$\MOD\ so any subset of $\vec{w}$ in the over-approximate abstract model is going to satisfy the \HP, so any subset of $\vec{W}$ in the concrete model is going to satisfy as well.
	%     \item [--] We need to show that \MU$\models [\vec{X}\leftarrow h_U^{-1}(\vec{x}),\vec{W}\leftarrow h_O^{-1}(\vec{w}), \vec{Z}'\leftarrow h_O^{-1}(\vec{z^*})]\neg h_U^{-1}(\varphi)$, that means that if we change any subset of $\vec{W}$ (other variables) in the abstract model it does not influence $h_U^{-1}(\varphi)$. As we know $O\geq$\MOD\ so any subset of $\vec{w}$ in the over-approximate abstract model is going to satisfy the \HP, so any subset of $\vec{W}$ in the concrete model is going to satisfy as well, it means that $\vec{w}$ in over-approximate model has the upper hand in the number of states compared to the concrete model \MOD. Therefore, if any change in a subset of the abstract model doesn't change the effect, and the concrete model is a subset of the abstract (over-approximate) model ($O\geq$\MOD), so in conclusion, if it works for the over-approximate model it is going to work for the concrete model.
	%     \item [--] $h_U^{-1}(\vec{x})$ may not be minimal in the concrete model, $\vec{x}$ is minimal in the abstract model, and we do care about the abstract model, not the concrete model cause we want to prove that cause in the abstract model contains the cause in the concrete model. In addition, we need to prove that $\vec{x}$ is minimal in the abstract model, to do so we remove one of the sets in $h_U^{-1}(\vec{x})$, now we need o prove that this is not cause in abstract model. 
	% \end{itemize}
% The relation between the over-approximate, under-approximate, and concrete model is shown, in \figref{f5}.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\linewidth]{images/f5.png}
	\caption{Schematic of the over-approximate, under-approximate, and concrete model.}
	\label{f5}
\end{figure}















% \newpage
% \textbf{First Proof} Suppose that $h^{-1}(x) = \langle z_i,z_j,\dots z_l\rangle$ and  $h^{-1}(\psi) = \langle z_i',z_j',\dots z_l' \rangle$, by definitions we know that some of the $<z_i,z_j,\dots z_l>$ and $<z_k,z_j,\dots z_m>$ may have same values. So any possible interventions on them are impossible. Suppose that there are $<z_i',z_j',\dots z_l> \in M \backslash h^{-1}(x)$ and $<z_k,z_j,\dots z_m> \in M \backslash h^{-1}(\psi)$ that satisfy HP and we do not consider them in the abstract model, this is impossible because if there are such these variables they would appear in GET\_CEX function so there is a contradiction and the theorem is proved. 
% \newline\textbf{Second Proof} Suppose that $h^{-1}(x) = <z_i,z_j,\dots z_l>$ and  $h^{-1}(\psi) = <z_i',z_j',\dots z_l'>$, by definitions of AC1 and AC2(b) if cause happens effect should happen and if the cause does not happen we can not observe the effect. So we assign all $<z_i,z_j,\dots z_l>$ to true. We have some changes in the $<z_i',z_j',\dots z_l'>$ then we assign all variables $<z_i,z_j,\dots z_l>$ to false, so we see some changes in $<z_i',z_j',\dots z_l'>$, in some variables we observe  $T\rightarrow T$ and $F\rightarrow F$ behavior and these variables are cause and effect of the concrete model (If there is no variable that has this behavior, we don't have cause and effect relation in the concrete model because there was a cause and effect we would add them in REFINE phase of the algorithm). In \figref{f2}, the model contains a couple of variables colored red, orange, blue, green, and white. each of these colors is the final concept of how the mapping function works.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\linewidth]{images/f3.png}
	\includegraphics[width=0.45\linewidth]{images/f2.png}
	\caption{Example describes the Algorithm}
	\label{f2}
\end{figure}
\newpage







\section{New Theory}
If a Causal structure in approximate models, $U$ and $O$, such that, 
\begin{itemize}
	\item[] $(U,\vec{u}) \models (\vec{X} = \Vec{x}_U) \varphi_U$ $\wedge$
	\item[] $(U,\vec{u}) \models (\vec{X} \leftarrow\Vec{x}'_U, \vec{W} \leftarrow \vec{w}_U) \neg\varphi_U$ $\wedge$
	\item[] $(O,\vec{u}) \models (\vec{X} \leftarrow\Vec{x}_O, \vec{W}' \leftarrow \vec{w}_O, \Vec{Z}' \leftarrow \vec{z}_O^*) \varphi_O$
\end{itemize}

\noindent then we have,

\begin{itemize}
	\item[] $(\mathcal{M},\vec{u}) \models (\vec{X} = h^{-1}_U(\vec{x}))h^{-1}_U(\varphi)$ $\wedge$ \todo{I don't like it}
	\item[] $ (\mathcal{M},\vec{u}) \models (\vec{X} \leftarrow h^{-1}_U(\vec{x}'), \vec{W}\leftarrow h^{-1}_U(\vec{w}_U))\neg h^{-1}_U(\varphi)$ $\wedge$
	\item[] $ (\mathcal{M},\vec{u}) \models (\vec{X} \leftarrow h^{-1}_O(\vec{x}'), \vec{W}'\leftarrow h^{-1}_O(\vec{w}_O),\vec{Z}' \leftarrow h^{-1}_O(\vec{z}^*_O))h^{-1}_O(\varphi)$
\end{itemize}

\noindent such that is true in the concrete model. 

\subsection{Proof}
To prove this Theorem we divide the problem into three subproblems,
\begin{itemize}
	\item [--] We need to show that $(\mathcal{M},\vec{u}) \models (\vec{X} = h^{-1}_U(\vec{x}))h^{-1}_U(\varphi)$, this is easy to see that if we find a cause and effect in under-approximate abstract, it is is going to be a cause for the concrete model, because in the definition of under-approximate abstract $U\leq $\MOD\ so it is impossible to find a causal relation in $U$ that is not true in \MOD.
	\item[--] We need to show that $ (\mathcal{M},\vec{u}) \models (\vec{X} \leftarrow h^{-1}_U(\vec{x}'), \vec{W}\leftarrow h^{-1}_U(\vec{w}_U))\neg h^{-1}_U(\varphi)$, so in other words counterfactual criterion under the \emph{contingency} $\vec{W}\leftarrow h_U^{-1}(\vec{w})$ in abstract model should be observed in concrete model. 
	%
	Same as the first item it is easy to show that if $h_U^{-1}(\vec{x})$ does not happen in the concrete model we are going to see $h_U^{-1}(\varphi)$, and also we need to show that any subset of $\vec{W}$ held constant at some setting $h_U^{-1}(\vec{w})$. 
	%
	As we know $U\leq$\MOD\ so some subset of $\vec{w}$ in the under-approximate abstract model is going to satisfy the \HP, so any subset of $\vec{W}$ in the concrete model is going to satisfy as well.
	
	\item [--] We need to show $ (\mathcal{M},\vec{u}) \models (\vec{X} \leftarrow h^{-1}_O(\vec{x}'), \vec{W}'\leftarrow h^{-1}_O(\vec{w}_O),\vec{Z}' \leftarrow h^{-1}_O(\vec{z}^*_O)) h^{-1}_O(\varphi)$, that means that if we change any subset of $\vec{W}$ (other variables) in the abstract model it does not influence $h_O^{-1}(\varphi)$. 
	%
	As we know $O\geq$\MOD\ so any subset of $\vec{W}$ in the over-approximate abstract model is going to satisfy the \HP, so any subset of $\vec{W}$ in the concrete model is going to satisfy as well, it means that $\vec{w}$ in over-approximate model has the upper hand in the number of states compared to the concrete model \MOD. 
	%
	Therefore, if any change in a subset of the abstract model doesn't change the effect, and the concrete model is a subset of the abstract (over-approximate) model ($O\geq$\MOD), so in conclusion, if it works for the over-approximate model it is going to work for the concrete model.
	
	
	\item [--] $h_U^{-1}(\vec{x})$ may not be minimal in the concrete model, $\vec{x}$ is minimal in the abstract model, and we do care about the abstract model, not the concrete model cause we want to prove that cause in the abstract model contains the cause in the concrete model. In addition, we need to prove that $\vec{x}$ is minimal in the abstract model, to do so we remove one of the sets in $h_U^{-1}(\vec{x})$, now we need o prove that this is not cause in abstract model. 
\end{itemize}









\section{Example}
In this scenario \figref{f4}, we have network with $s1,s2,s3,s4,s5,s6$ nodes and links $e1,e2,e3,e4,e5,e6$. The source of our network is s1 and data should use the links and nodes to reach s6, imagine all the nodes are working well, but we might have a failure in the links, so the expression that defines it would be $s6 = (e1\wedge e4 \wedge e5)\vee (e2\wedge e4 \wedge e6)$. We want to find an abstraction that preserves the HP, starting with finding \textbf{A}, in the first iteration take e1 as the first element $A={e1}$ then we check for MMC we see when we make it true or false s6 is unknown. and we ask for any counterexamples, GET\_CEX return e6 that, now we add s6 to A, $A={e1,e6}$, the process goes for some more iteration and we have $A={e1,e6,e2,e4}$, Now MMC returns true. and based on HP we know that $cause={e1,e6,e4}$ is true. So A has part of the contains the cause and it is smaller, and the abstraction function is subjective and we do not change any interventions. 

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.5]{images/f4.png}
	\caption{Network Example}
	\label{f4}
\end{figure}






\section{Ideas about Probabilistic Causal Models}
In \figref{f1} we have a concrete model contains states $s_1,s_2,s_3,s_4$ and abstract model $S1,S2$ , imagine $s_1,s_2,s_3$ are possible causes for $s_4$. Our transitions can be computed as $\frac{p_i}{p_1,...,p_j}$, $p_1,...,p_j \in S_i$. So for our example, $s_1-s_4=0.4$, $s_2-s_4=0.26$, $s_3-s_4=0.33$, so for each, we have new transition probabilities.
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.4]{images/f1.png}
	\caption{Probabilistic Abstraction}
	\label{f1}
\end{figure}
\newpage
\section{exmaple}
The general formula for the electric potential energy of a system of point charges is given by:

\[ U = \sum_{i=1}^{n} \sum_{j=i+1}^{n} \frac{k \cdot q_i \cdot q_j}{r_{ij}} \]

Where:
- \(U\) is the electric potential energy,
- \(k\) is Coulomb's constant,
- \(q_i\) and \(q_j\) are the magnitudes of the charges,
- \(r_{ij}\) is the separation between charges \(i\) and \(j\).

This formula involves \(n\) charges, resulting in \(n(n-1)/2\) terms, each with three variables.

For example, consider the case where you have two point charges \(q_1\) and \(q_2\) separated by a distance \(r\). In this case, the formula can be simplified to:

\[ U = \frac{k \cdot q_1 \cdot q_2}{r} \]


% \section{Example}
% In quantum physics, let's consider the wavefunction (\(\Psi\)) for a particle described by the Schrödinger equation. The general form of the time-independent Schrödinger equation is:

% \[ \hat{H} \Psi = E \Psi \]

% Where:
% - \(\hat{H}\) is the Hamiltonian operator,
% - \(\Psi\) is the wavefunction of the particle,
% - \(E\) is the energy eigenvalue.

% The Hamiltonian operator involves kinetic and potential energy terms, and the wavefunction \(\Psi\) depends on the spatial coordinates of the particle.

% To abstract and simplify, let's consider the case of a particle in a one-dimensional box. In this scenario, the Hamiltonian operator is simpler, and the Schrödinger equation becomes:

% \[ -\frac{\hbar^2}{2m} \frac{d^2\Psi}{dx^2} = E \Psi \]

% Here:
% - \(\hbar\) is the reduced Planck constant,
% - \(m\) is the mass of the particle,
% - \(x\) is the spatial coordinate.

% This abstracted form captures the essential nature of the Schrödinger equation for a particle in a one-dimensional box, providing insight into the quantization of energy levels for confined systems in quantum mechanics.

% \section{Example}
% Certainly! Let's consider the formula for the time evolution of a quantum state, particularly the time-dependent Schrödinger equation. The general form of the time-dependent Schrödinger equation is given by:

% \[ i\hbar \frac{\partial \Psi}{\partial t} = \hat{H} \Psi \]

% Where:
% - \(i\) is the imaginary unit,
% - \(\hbar\) is the reduced Planck constant,
% - \(\Psi\) is the wavefunction,
% - \(\hat{H}\) is the Hamiltonian operator representing the total energy of the system,
% - \(\frac{\partial \Psi}{\partial t}\) is the partial derivative of the wavefunction with respect to time.

% This formula involves complex numbers and operators. However, it can be abstracted and simplified for a non-relativistic, single-particle system with a time-independent Hamiltonian. In this case, the time-dependent Schrödinger equation becomes:

% \[ i\hbar \frac{\partial \Psi}{\partial t} = -\frac{\hbar^2}{2m} \nabla^2 \Psi + V(\mathbf{r})\Psi \]

% Here:
% - \(m\) is the mass of the particle,
% - \(\nabla^2\) is the Laplacian operator representing spatial derivatives,
% - \(V(\mathbf{r})\) is the potential energy as a function of position.

% This abstracted form captures the time evolution of the quantum state for a non-relativistic particle in a potential field, and it is a fundamental equation in quantum mechanics.

\fi


==> letter.tex <==
\begin{center}
	{\bf \large Response Letter}
	\end{center}
\vspace{-1mm}		

We deeply thank all the reviewers for their constructive and insightful feedback. Guided 
by the suggestions and questions, we have significantly enhanced the content, focusing on resolving 
ambiguities and highlighting the application of our approach in the CPS domain and its impact on 
engineering safety-critical systems. We did our best to address all the comments and questions 
raised by the reviewers. 
Below, we elaborate on comments in the meta review and those by individual reviewers and detailed 
responses and clarifications to address the questions and concerns raised by the reviewers. We 
highlighted the modified parts using \revision{\bf red color}. 

Before we delve into our responses, we note that since there were no issues raised about the proof 
of Theorem~\ref{thrm:soundness}, we removed the proof from Section~\ref{sec:absref} to open 
space for more crucial parts, especially Sections~\ref{sec:eval} and~\ref{sec:causalanalysis}. If the 
paper is accepted, we will make the proof available on {\small \sf arXiv.org} or purchase an additional 
page (if there is such an option).

%\vspace{-1mm}		
\begin{center}
\textsc{\underline{Comments in the Meta Review}}
\end{center}

%We first answer the comments in meta review.\\

 {\em --- ``The empirical results are evaluated on {\bf \em two toy examples} (lunar lander and 
 mountain 
	car). The framework may be more convincing if the approach works for some non-toy and 
	non-neural network/reinforcement learning system.''} \\

\vspace{-2mm}		
We significantly expanded our experimental evaluation. First, we added a new case study (now in 
the new Section~\ref{sec:f16}) on an MPC-based controller (as suggest in the reviews to include a 
non-AI controller) for an F-16 autopilot simulator based on the work 
in~\cite{ARCH18:Verification_Challenges_in_F_16}. This 
case study itself has two scenarios where safety can be failed and we explain the root-cause of 
failures. We also made our Lunar Lander case 
study more complex by (1) adding more variables that contribute to the behavior of the controller 
(i.e., gravity, wind, and turbulence power), and (2) training 576 new neural networks (taking 6 
days to complete) and collecting 82,000 more traces. This experiment now clearly shows the limits 
of our SMT-based solution which times out after 20000 traces while our abstraction-based 
technique can handle 82,000 traces in a matter of four minutes. All details are added to 
Section~\ref{sec:eval}. \\

\vspace{-2mm}		
 {\em --- ``Section V.F links back to the original motivation of the approach, which is great, but this 
 could be significantly expanded to better {\em \bf demonstrate the benefits}…. If we just simulated 
 this (let's say monte carlo) and take the control inputs, would we find the failures? {\bf \em What 
 does the causality approach really add}?''}\\

\vspace{-2mm}		

First, please note that the objective of our technique is {\em not} to find failures. The goal of 
causality analysis is to {\em explain} why exactly they happened and how counterfactual scenarios 
would avoid them. 
Simulation (let's say monte carlo), verification, and testing may identify failures, but they do not 
explain why they happened. For example, Fig.~\ref{fig:tarce} shows the causal reason for violation safety in the 
mountain car example is a very early bad decision by the controller (i.e., $\action(0)=1$), where we 
prove that in the absence of this decision safety would have been violated (example added at the 
end of Section~\ref{sec:pre}). Finding such an explanation has been a long-standing and very 
challenging problem for different reasons from formal treatment of causal effect of events to the 
computational 
complexity of counterfactual reasoning. We added a paragraph to the introduction to explain the real 
objectives of our work.
Secondly, as rightly suggested by the reviewers, we substantially expanded the old Section V.F 
(now, Section~\ref{sec:causalanalysis}) in terms of how our approach assists in identifying the cause 
of safety violations and explains why they happened. For example, Figs.~\ref{fig:f16_analysis} 
and~\ref{fig:f16_analysis_counter} show real failed and counterfactual (successful) trajectories of 
the F-16 controller identified by our technique\\

\vspace{-2mm}		

{\em --- ``The presentation of the causality framework is {\bf \em challenging for this 
community}.''}\\
\vspace{-2mm}		

 We understand the challenge and this is exactly why we are very excited about the novelty of our 
work and presenting our findings to the EMSOFT audience. We strongly believe this paper brings a 
new and quite useful technique to the community which will open 
new research avenues, especially benefiting the industrial efforts to develop safety-critical systems. 
We have added more soft text to the paper to explain the concepts better. We also understand there 
is (perhaps) heavy notion and symbols involved, but they have to be kept to ensure mathematical 
rigor of our results.

\vspace{-1mm}		
\begin{center}
	\textsc{\underline{Response to Individual Reviewers}}
\end{center}

\vspace{-1mm}		
\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm]
\footnotesize
{\bf Reviewer A:} What your algorithm provides as an answer and whether that's useful. For example, with 
the lunar lander, did it actually identify cases where it had made the wrong choice and you can show 
that this led to it landing incorrectly?
\end{tcolorbox}
\vspace{-1mm}		
%
\noindent {\bf Response:} Indeed, this is the case. We have substantially revised 
Section~\ref{sec:causalanalysis}, added another case study, and explained the outcome of our 
technique in greater detail. For example, our technique explains the reason for failure of lunar lander 
is when there is strong wind from left to right, the lander tends to overuse its right engine. Also, the 
newly 
added Figs.~\ref{fig:f16_analysis} and~\ref{fig:f16_analysis_counter} also show real failed aircraft 
trajectory and the corrected one based on the counterfactual scenario using our technique.

\vspace{-1mm}		
\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm]
\footnotesize {\bf Reviewer A:} Whether your sets of variables were finite… I presume that using an 
SMT solver restricts your solutions to finite sets of variables, but you don't seem to ever mention 
this.
\end{tcolorbox}
\vspace{-1mm}		
%
\noindent {\bf Response:} This is not true. SMT solvers {\em can} handle theories with 
infinite-domain variables (e.g., integers, reals, etc). 

\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm]
	\footnotesize {\bf Reviewer A:} Do you actually incorporate the details of the controller into the model seen 
	by the SMT solver, or its its behavior somehow hidden across a variety of traces with different initial 
	conditions?
\end{tcolorbox}
%
\noindent {\bf Response:} Yes. Our solution may take as input the model of a controller as a transition 
system. This is a general way to model the behavior of any system. Or, it can be agnostic to the details of 
the controller and take a set of execution traces. We clarified this in the first paragraph of
Section~\ref{sec:smt}.

\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm]
	\footnotesize {\bf Reviewer A:} Since these traces of time series and the controllers necessarily don't look 
	forward in 
time, can the SMT solver or something else take advantage of that form of causality? Part of my 
confusion is that when I see causality, I immediately think of temporal causality.
\end{tcolorbox}
%
\noindent {\bf Response:} 
As mentioned in Section~\ref{sec:pre}, please note that in the \HP framework, causal models 
are ``recursive”: given a context, there are no cyclic dependencies. A temporal causality loop is a 
type of phenomenon whereby a specific moment in time repeats itself continually inside an 
independent fragment of time. This paper, is not concerned with causality loops.

\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm]
	\footnotesize {\bf Reviewer A:}  ...whether this technique is practical for any real-world example? 
	The experiments you conducted seem like toys.
\end{tcolorbox}
%
\noindent {\bf Response:} 	
Root-cause analysis of safety failures has been in the interest of academic as well as 
industrial circles for decades. This problem is much harder than finding ``bugs” and is concenred with 
{\em explaining} the underlying reason of failures happening. Our work is the first step in automating 
discovery of actual cause 
of failures and our experiments show that we are able to identify earliest bad decisions by controllers 
that lead violation of safety requirements. We have elaborated on this in the introduction (see first 
and last paragraphs of the introduction). 
%
In terms of experiments, we have substantially expanded them in two fronts. First, we added a new case 
study on (now in Section~\ref{sec:f16}) on a non-AI MPC-based controller for an F-16 autopilot 
simulator. This 
case study itself has two scenarios where safety can be failed. Secondly, we made our Lunar Lander 
case study more complex by (1) adding more variables that contribute to the behavior of the controller 
(i.e., gravity, wind, and turbulence power), and (2) training 576 new neural networks (taking 6 
days to complete) and collecting 80,000 more traces. This experiment now clearly shows the limits 
of our SMT-based solution which times out after 20000 traces while our abstraction-based 
technique can handle 80,000 traces in a matter of four minutes. All details are added to 
Section~\ref{sec:eval}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=red!8!white]
	\footnotesize {\bf Reviewer B:}  The paper thoroughly discusses the use of the Z3 SMT solver but mentions 
	another solver only briefly as "a search technique commonly used in data analysis," referencing 
	libraries [23] and [22]. It would be beneficial for the paper to describe this second solver in greater detail..
\end{tcolorbox}
%
\noindent {\bf Response:} Thanks for your comment. We addressed this ambiguity in the 4th 
paragraph of Section~\ref{sec:impl}. In summary, Z3 is used for solving problems with symbolic 
constraints. However, our problem can be transformed into a search problem if there is no symbolic 
logic for infinite-domain variables are present, where we are looking for traces that satisfy our 
constraints. Therefore, because we are working with large datasets of traces, we employ search 
methods that are commonly used in the data analysis field.

\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=red!8!white]
	\footnotesize {\bf Reviewer B:}  There appears to be a lack of detailed results or analysis 
	demonstrating how effectively the approach identifies causal actions that lead to 
	successful/unsuccessful landings or destinations - which is a main objective of the paper. If the graphs 
	primarily plot the number of traces against time without distinguishing between successful and 
	unsuccessful outcomes (i.e., successful vs. unsuccessful landings/destinations), it remains unclear 
	how the causal analysis has enhanced the success rate of these traces and how well the method is 
	identifying causal actions. Providing clarification or additional results that explicitly link the causal 
	analysis to improvements in operation success would significantly bolster the paper's assertions that 
	they can identify actual causes in a computing system.
\end{tcolorbox}
\noindent {\bf Response:} Thank you for your comment. We completely agree and have added 
text to the revised version in the first part of Section~\ref{sec:impl} to clarify the ambiguity about traces 
and the success and failure rate. To address the second part of your comment, we should emphasize 
that our technique currently only finds actual cause of effects and explains them. It can also produce 
counterfactual scenarios that lead to success. However, it doesn't automatically 
repair them. That's why it cannot characterize changing success rate. But it can be used to manually 
repair the causal reason of failures. In other words, 
	if we identify a cause in a failure trace, it means there is a counterfactual scenario that leads to 
	success. By using the counterfactual decision, the trace will result in success. Additionally, in the 
	revised Section~\ref{sec:causalanalysis}, we elaborate on this observation more thoroughly in 
	Section~\ref{sec:eval}. The newly added Figs.~\ref{fig:f16_analysis} 
	and~\ref{fig:f16_analysis_counter} specifically show real failed aircraft trajectory and the 
	corrected one based on the counterfactual scenario using our technique.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=red!8!white]
	\footnotesize {\bf Reviewer B:}  I would need to see more results on how well their method identifies 
	actual causes in a computing system to be confident in their method.
\end{tcolorbox}
\noindent {\bf Response:}
We completely agree with your comment. Consequently, we have added one more case study 
(F-16 autopilot controller in Section~\ref{sec:f16}) and expanded our Lunar Lander experiment to the 
limit of our computational power during the revision period, as training multiple networks and 
generating traces is time-consuming. 
Our F-16 simulation case study (especially the newly added Figs.~\ref{fig:f16_analysis} 
and~\ref{fig:f16_analysis_counter}), which is a non-AI (MPC controller) experiment, demonstrates 
the scalability and significance of our approach in identifying the causes of failures in cyber-physical 
systems. Additionally, we have significantly expanded Section~\ref{sec:causalanalysis} and 
thoroughly explained how our results assists in explaining the actual cause of safety violations in 
CPS.


%\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=red!8!white]
%	\footnotesize {\bf Reviewer B:}  Detailed comments.
%\end{tcolorbox}
%\noindent {\bf Response:} Thank you for your careful reading of the paper. We fixed all the errors.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=blue!8!white]
	\footnotesize {\bf Reviewer C:}  Section V.F could be more developed, as it is the main result of the 
	article.
\end{tcolorbox}
\noindent {\bf Response:} We completely agree with your observation. We first added a new 
case studty (F-16 MPC autopilot controller in Section~\ref{sec:f16}) and then elaborates on the 
analysis. We aim to show how 
identifying the root causes of failures can benefit the community. We also substaintially expanded 
Section~\ref{sec:causalanalysis} and discuss how (when a failure occurs) counterfactual scenarios 
(alternative decisions under the same conditions that lead to success) helps pinpoint the poor 
decisions that caused the failure. In the revised Section~\ref{sec:causalanalysis}, we now describe 
how the root 
reason of failures and show how caounterfactual scenrios would lead to satisfaction of the specification.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=blue!8!white]
	\footnotesize {\bf Reviewer C:} The introductory example of Coulomb's law is neither clear nor helpful.
\end{tcolorbox}
\noindent {\bf Response:} We agree and removed this example.



\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=blue!8!white]
	\footnotesize {\bf Reviewer C:} Section~\ref{sec:TS} hard to follow, with too many symbols.
\end{tcolorbox}
\noindent {\bf Response:} We understand that this section is a bit heavy on notation and math. This is 
necessary to ensure mathematical rigor of our algorithm and the proof of correctness. Unfortunatley, for 
reasons of space and the fact that we have significantly expanded other sections to show the 
benefits of 
our approach, we could not add more text to this section. 


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=blue!8!white]
	\footnotesize {\bf Reviewer C:} No complexity analysis of the algorithm is made.
\end{tcolorbox}


\noindent {\bf Response:} In the introduction, we already did mention that the decision problem for 
identifying actual causality in a causal model is {\sf \small DP-complete}. This is, for example, similar 
to solving integer linear programs, which is an {\sf \small NP-complete} problem and heuristic 
algorithms only attempt to solve 
the problem more efficiently (compared to a brute-force solution) but that does not change the 
complexity class. We added some text to the last paragraph of Section \ref{sec:smt} and the 
paragraph before Section~\ref{sec:TS}.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=blue!8!white]
	\footnotesize {\bf Reviewer C:} In introduction, the $\varphi_{\mathsf{hp}}$ formula is 
	incomprehensible without more context
\end{tcolorbox}
\noindent {\bf Response:} We added more text to the description of the formula to explain it better in the introduction.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=blue!8!white]
	\footnotesize {\bf Reviewer C:} In Fig 4, you could say why trace $\tau_0$ and $\tau_2$ are the same. 
	We discover it only a few sections later.
\end{tcolorbox}
%
\noindent {\bf Response:} Thank you for your comment. We added more explanations to 
Example~\ref{ex:car_explain}. In summary, in this example, the set $\vec{W}$ is empty, which 
means 
that {\bf AC2(b)} is 
equivalent to {\bf AC1}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=green!8!white]
	\footnotesize {\bf Reviewer D:} This is a bit misleading, because I would expect some contributions at 
	the level of causality theory, but actually the technical contribution of this paper is about the cases in 
	cyber-physical systems.
\end{tcolorbox}
%
\noindent {\bf Response:} Unfortunately, we don’t quite understand what is misleading here. We never 
claimed contributions towards the theory of causality or a new definition/notion of causality. We do 
mention in several places we are motivated by the \HP definition and we propose a way to discover 
actual causes and we demonstrate its application in safety of CPS. We rewrote parts of the abstract and 
introduction to reflect this point.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=green!8!white]
	\footnotesize {\bf Reviewer D:} In Section II the preliminaries, I don’t see a clear description about the 
	CPS model under consideration, but instead, it is given as a by-product of causality model. While it’s 
	nice to know the details of the general causality model, I would prefer to see how it is applied as a tool 
	to solve the problems in the context of CPS. (think of removing Sec 2)
\end{tcolorbox}
%
\noindent {\bf Response:}  Thank you for this comment. Interestingly, we have gone back and forth on 
including/excluding Section~\ref{sec:pre} several times from the moment we started writing the paper. 
We totally appreciate your suggestion. We finally decided to keep it (again) to make sure (1) the paper is 
self-contained, and (2) the reader has access to the baseline definitions of the \HP frameowrk to 
understand how we formalized \HP in Fig. \ref{fig:HP}. Also, please note that in the \HP framework, 
structural equations can model how a CPS model works. Likewise, in our setting we use transition 
systems which are pretty general in modeling computing systems, including CPS. We added a 
comment on this in the beginning of Sections~\ref{sec:pre} and~\ref{sec:smt}.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=green!8!white]
	\footnotesize {\bf Reviewer D:} Regarding the cause event $\varphi_c$ and effect event $\varphi_e$, I 
	wonder how they are formalized in the technique. Are they manually formalized by users?
\end{tcolorbox}
%
\noindent {\bf Response:}  Please note that Section~\ref{sec:causal_form} introduces the notion of causal 
formulas, which are used to formalize $\varphi_c$ and $\varphi_e$. In Example~\ref{ex:setting}, we 
have:
$$
\varphi_\fail = \pos(n) \neq 0.6
$$
where $0.6$ is the flag position and $n$ is the last state of the car. This is a simple 
safety condition and can be obtained by the user, a failed test case, or a model checker. We added a 
sentence in the 
beginning of Section~\ref{sec:causal_form}  to clarify 
this. How $\varphi_e $ is found is irrelevant to the problem studied in this paper. We also clarified 
this in the ``{\tt tcolorbox}" in the introduction (it is also reflected in the SMT Decision problem in 
Section~\ref{sec:smt}).


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=green!8!white]
	\footnotesize {\bf Reviewer D:}  Second, the formulas in Fig.~\ref{fig:HP} that contain temporal 
	operators, cannot be directly solved as constraints by SMT solvers, right? If I’m correct, the translation 
	from these formulas to SMT constraints is not trivial, but the details are not shown in the paper.
\end{tcolorbox}
%
\noindent {\bf Response:}  Thank you for your comment. This translation is relatively trivial. We moved some text around in Section~\ref{sec:smt-form-ac} and added more explanation to clarify the SMT constraints, in particular, the temporal operators. The short answer is while SMT solvers cannot directly encode temporal operators, one can easily encode them using the above expanded definitions by quantifiers over traces, which we added in Section Section~\ref{sec:smt-ts}.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=green!8!white]
	\footnotesize {\bf Reviewer D:} I don’t know in the context of this paper, e.g., how an 
	over-approximate system $\hat{\mathcal{T}}$ is constructed, or how it is refined based on a 
	counterexample.
\end{tcolorbox}
%
\noindent {\bf Response:}  Please note that the construction of the over-approximation model is 
already explained in the 4th paragraph of Section~\ref{sec:impl}. We also illustrate this process 
using a simple example from the Mountain Car problem.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=green!8!white]
	\footnotesize {\bf Reviewer D:}  Moreover, the formulas in Fig.~\ref{fig:HP} , which is a main technical 
	contribution in the paper that instantiates the actual causality conditions, do not seem too difficult to 
	build. I’m not sure how much effort is needed in order to build them, or what is the main technical 
	difficulty when building them.
\end{tcolorbox}
%
\noindent {\bf Response:}  Indeed, building these formulas is not particularly difficult. This is the first step 
to reason about the \HP definition of actual causality in computing systems modeled  as a transition 
systems. It sets the stage for an SMT solution and subsequently our abstraction-refinement techniqe.


\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=green!8!white]
	\footnotesize {\bf Reviewer D:} It seems that the encoding Fig.~\ref{fig:HP} is sound but not complete, 
	and the authors also recognize it. Regarding this point, I would expect more analysis on what is 
	missing.
\end{tcolorbox}
%
\noindent {\bf Response:} No. The SMT-based solution (including formulation of HP in 
Fig.~\ref{fig:HP} ) is sound {\em and} complete. The abstraction-refinement is sound but not 
complete because it is a heuristic (similar to the well-known CEGAR approach in model checking). 
We added some text to the introduction as well as Sections~\ref{sec:smt} and \ref{sec:absref} to 
explain this.



\begin{tcolorbox}[boxrule=.5pt,boxsep=-1mm,colback=green!8!white]
	\footnotesize {\bf Reviewer D:} Minor issues: The first line of Section~\ref{sec:smt}: “transom” should 
	be “transform” Use different equal marks to differentiate different cases, e.g., assignment and 
	equivalence between formulas.
\end{tcolorbox}
%
\noindent {\bf Response:} This is now fixed and we switch to $\triangleq$ wherever we define Boolean predicates.










%

%\begin{center}
%	\textsc{\underline{Major Changes}}
%\end{center}
